Variability Fault Localization: A Benchmark

Software fault localization is one of the most expensive, tedious, and time-consuming activities in program debugging. This activity becomes even much more challenging in Software Product Line (SPL) systems due to the variability of failures in SPL systems. These unexpected behaviors are caused by variability faults which can only be exposed under some combinations of system features. Although localizing bugs in non-configurable code has been investigated in-depth, variability fault localization in SPL systems still remains mostly unexplored. To approach this challenge, we propose a benchmark for variability fault localization with a large set of 1,570 buggy versions of six SPL systems and baseline variability fault localization performance results. Our hope is to engage the community to propose new and better approaches to the problem of variability fault localization in SPL systems.

==> background.tex <==
\section{Background}
\label{section:background}
\input{testing}
\input{varbugs}
\input{fault_localization}


==> fault_localization.tex <==
\subsection{Fault Localization}

\begin{itemize}
    \item adaption (state of the art -> SBFL)
    \item 2 reasons why this adaption is wrong (contribute differently \& test case incompatibility) (see submitted papers)
    \item test quality (passing product still contains bugs because the tests couldn't uncover any of them)
    
\end{itemize}

==> testing.tex <==
\subsection{Testing in Software Product Lines}
%
The software product line approach provides a form of mass customization by constructing individual solutions based on a portfolio of reusable software components called \textit{features} \cite{?}. \textit{Feature} is an optional or incremental unit of functionality \cite{?}. A \textit{feature model} documents the features of a product line and their relationships. Taking advantage of feature modularity, an SPL system create a growing set of different \textit{products} by combining \textit{features} based on various \textit{configurations} \cite{?}.

%
\textit{Feature interactions} are the communications between two or more features when they are all involved to produce a new product. In other words, a feature interaction occurs when a feature behavior is influenced by the presence of another features \cite{?}. Previous researches reports existing faults caused by unintended feature interactions, which impossible to detect when analyzing each of features individually. This issue becomes more problematic when potential feature interactions can increase exponentially with the number of features.

%
Currently, most of the techniques for testing and debugging software product lines are still performed individually with respect to each product. Thus, verifying all the interactions occurred in an SPL system is nearly infeasible in practice. To reduce cost of failures revealed by unexpected feature interactions, prior work \cite{?} devise Combinatorial Interaction Testing (CIT) approach, which samples only small combinations of features for testing purpose. This technique introduces the notion of t-wise coverage, which is the condition that achieves all combinations of t features and generate minimum configuration space. Actually, developers often apply the common values t in range from 1 to 5 \cite{?} to ensure its scalability in real-world SPL systems.

%
Furthermore, the enrichment of test cases to satisfy a testing criterion also raises a complex task to be solved in SPL field \cite{?}. At the moment, the common way to verify sampled products is to derive traditional techniques and generate test suite for each of products individually.

==> varbugs.tex <==
\subsection{Variability Bugs}
\begin{itemize}
    \item phenomena
    \item root cause, potential cause \& effect
\end{itemize}
